Delayed approximate matrix assembly in multigrid with dynamic precisions

The accurate assembly of the system matrix is an important step in any code that solves partial differential equations on a mesh. We either explicitly set up a matrix, or we work in a matrix-free environment where we have to be able to quickly return matrix entries upon demand. Either way, the construction can become costly due to non-trivial material parameters entering the equations, multigrid codes requiring cascades of matrices that depend upon each other, or dynamic adaptive mesh refinement that necessitates the recomputation of matrix entries or the whole equation system throughout the solve. We propose that these constructions can be performed concurrently with the multigrid cycles. Initial geometric matrices and low accuracy integrations kickstart the multigrid, while improved assembly data is fed to the solver as and when it becomes available. The time to solution is improved as we eliminate an expensive preparation phase traditionally delaying the actual computation. We eliminate algorithmic latency. Furthermore, we desynchronise the assembly from the solution process. This anarchic increase of the concurrency level improves the scalability. Assembly routines are notoriously memory- and bandwidth-demanding. As we work with iteratively improving operator accuracies, we finally propose the use of a hierarchical, lossy compression scheme such that the memory footprint is brought down aggressively where the system matrix entries carry little information or are not yet available with high accuracy.

==> 06_integration.tex <==
\section{Integration}
\label{section:integration}

We speak about the integration into one solver here


Header mit laenge des Stencils
hierarchische Kompressions
\marginpar{Disable coarse grids -> remark; this could be a premature coarse
grid disable} 


\marginpar{Shall we refer to the non-diagonal dominance thing here?}


Two streams for two precision.
Extension straightforward
Marker per cell


Define starvation

Let each vertex hold its $\mathbf{A},\mathbf{P}$
and $\mathbf{R}$ contributions twice.
$\mathbf{A},\mathbf{P},\mathbf{R}$ are the actual values used by the solver.
$\mathbf{A}^{new},\mathbf{P}^{new},\mathbf{R}^{new}$ are helper variables.

\subsection{Lazy evaluation}

In a Haskell sense
Different to previous paper
Special flavour of paradigm where we wait



\subsection{Hotness}

Ways to avoid that: Some level of ``hotness'' where see if stencil element is troubled and hold off updating if that happens; if stencil slow converging then be more aggressive with how increase size of quadrature.


Cartoons added?
Source code added?
Alles vom alten Paper mit drin?

\subsection{Non-linear equations}

Wenn sich massiv was aendert, muessen wir es bottom-up hochpropagieren





We have not yet
computed the cell's contribution towards any stencil.
If $p(c)=\top$, the cell's contributions towards 
$\mathbf{A},\mathbf{P},\mathbf{R}$ 
are sufficiently accurate.
If neither condition is met, 
$\mathbf{A},\mathbf{P},\mathbf{R}$ hold an operator representation which results
from a subsampling of $c$ with a $p(c) \times p(c)$ quadrature.

%\input{algorithm-greedy-integration}

It is straightforward to phrase the assembly of the stencils, i.e.~the 
entries of $\mathbf{A}$, iteratively, and to fuse it with the mesh traversal
evaluating the multigrid's mat-vecs.
Such a fusion ensures that the assembly does not introduce additional data reads
and writes compared to the mat-vecs.
It releases pressure from the memory interconnect:
%
%
If a cell holds $\bot $, the grid has just been created due to $\mathcal{U}$
or this is the initial iterate.
The cell belongs to the fine grid.
In this case, we set $p=1$, compute the cell's contribution towards $\mathbf{A}$
and continue.
This is the initial instantiation of one task of $\mathcal{A}$ for one cell.
If we encounter a cell with $p \not= \top$, we increase $p$ by
one and recompute the cell's contribution towards $\mathbf{A}$.
The recomputed cell contributions are stored in $\mathbf{A}^{new}$.
We can then compare the relevant entries of $\mathbf{A}$ and $\mathbf{A}^{new}$.
If the entries' maximum difference is below $dp$, we set $p = \top$.
Finally, we roll over $\mathbf{A}^{new}$ into $\mathbf{A}$ to make it available
to the solver.
With this scheme, $\mathcal{A}_h(v)$ becomes a set of tasks 
parameterised though $p$.



%\input{algorithm-HTMG}
%
%
We augment each cell with one further atomic boolean which is unset initially.
Our greedy stencil integration then is formalised as follows.
If we encounter a fine grid cell with
%
%
\begin{enumerate}
  \item $p = \bot$, we run the integration as sketched above. This yields
  a low accuracy ``kick-off'' integration of the system matrix.
  \item $p = \top$, we do not alter the stencil.
  \item $p \not= \bot$ and  $p \not= \top$ whose atomic boolean
  is not set, we set the marker and spawn a new integration task running one
  adaptive integration as described above. It has low priority. Upon completion,
  the task unsets the marker.
  \item $p \not= \bot$ and  $p \not= \top$ whose atomic boolean
  is set, we continue.
\end{enumerate}  

\noindent
These steps integrate easily into any multigrid code.
The mat-vecs kick off with a low accuracy integration of
(\ref{equation:lazy:integration}) but create additional tasks that improve this
accuracy.
We postpone the accurate integration.
Standard multicore work stealing ensures that idling cores take over the
integration, i.e.~the matrix ``assembly'' branches out (Fig.~\ref{figure:lazy:illustrative}).


We assign each cell a 
What the quadrature is and what we're constructing

\begin{equation}
 \int _{\Omega _h} \epsilon \left( \nabla u, \nabla \phi \right) \ dx
  = 
 \sum _{c \in \Omega_h}
 \int _{c} \epsilon \left( \nabla u, \nabla \phi \right) \ dx,
 \label{equation:lazy:integration}
\end{equation}


